Quantum Cloning and Deletion in Quantum Information Theory

Quantum mechanics put restriction on performing some task which we can do classically. One such restriction is that we cannot copy an arbitrary quantum state. This is known as No-cloning theorem. Although quantum mechanics forbid us to construct a perfect cloner, there is no restriction to construct an imperfect cloner. Therefore, we have constructed and studied a special kind of quantum cloning machine named as Hybrid quantum cloning machine which is nothing but a different combination of pre-existing quantum cloning machines. We showed that this hybrid quantum cloning machine sometime gives better quality copy than the pre-existing quantum cloners. Quantum entanglement is a very astonishing property in a multi-partite system and it is a very useful ingredient of quantum information theory. Therefore broadcasting (cloning) of entanglement is a very important subject to study. In this regard we have studied the broadcasting of entanglement using state dependent quantum cloning machine. Further, we have investigated the problem of secretly broadcasting of three-qubit entangled state between two distant partners. Linearity of quantum mechanics put another restriction on deletion of an arbitrary quantum state i.e. an arbitrary quantum state against a copy cannot be perfectly deleted. Like cloning machine one can construct an approximate deletion machine also. Therefore, we have constructed an universal deletion machine in the sense that the fidelity of deletion does not depend on the input state and showed that the fidelity of deletion is 3/4 . Further we showed that the fidelity of deletion depends on the blank state at the output and it can be improved from the value 3/4 for certain blank state. Moreover, we have studied the case where two cloned copies are given at the input of the deletion machine.

==> chap15.tex <==
\large \baselineskip .85cm \setcounter{page}{127} \markright{\it
CHAPTER~\ref{chap7}. Bibliography}
\label{chap7}%
%
\begin{thebibliography}{99}
\bibitem{adhikari1} Adhikari, S., B.S.Choudhury, J. Phys. A: Math. Gen. \textbf{37}, 1 (2004).
\bibitem{adhikari2} Adhikari, S., Phys. Rev. A \textbf{72}, 052321 (2005).
\bibitem{adhikari3} Adhikari, S., B.S.Choudhury, I.Chakrabarty, J. Phys. A: Math. Gen. \textbf{39}, 8439 (2006).
\bibitem{adhikari4} Adhikari, S., B.S.Choudhury, Phys. Rev. A \textbf{73}, 054303 (2006).
\bibitem{adhikari5} Adhikari, S., B.S.Choudhury, Phys. Rev. A \textbf{74}, 032323 (2006).
\bibitem{azuma1} Azuma, K., J.Shimamura, M.Koashi and N.Imoto, Phys. Rev. A \textbf{72}, 032335 (2005).
\bibitem{audenaert2} Audenaert, K., F.Verstraete, T.D.Bie and B.D.Moor, e-print quant-ph/0012074.
\bibitem{audenaert1} Audenaert, K.M.R and J.Eisert, J. Math. Phys. \textbf{46}, 102104 (2005).
\bibitem{banaszek1} Banaszek, K., Phys. Rev. Lett. \textbf{86}, 1366 (2001).
\bibitem{bandyopadhyay1} Bandyopadhyay, S. and G.Kar, Phys. Rev. A \textbf{60}, 3296 (1999).
\bibitem{barnum1}  Barnum, H., C.M.Caves, C.A.Fuchs, R.Jozsa and B.Schumacher, Phys. Rev. Lett. \textbf{76}, 2818 (1996).
\bibitem{bennett1} Bennett, C.H., and G.Brassard, Proceedings of IEEE International
Conference on Computers, System and Signal Processing, Bangalore,
India, 1984, pp.175-179.
\bibitem{bennett2} Bennett, C.H., and S.J.Weisner, Phys. Rev. Lett. \textbf{69}, 2881 (1992).
\bibitem{bennett5} Bennett, C.H., Phys. Rev. Lett. \textbf{68}, 3121 (1992).
\bibitem{bennett3} Bennett, C.H., G.Brassard, C.Crepeau, R.Jozsa, A.Peres and W.K.Wootters,
Phys. Rev. Lett. \textbf{70}, 1895 (1993).
\bibitem{bennett4} Bennett, C.H., H.J.Bernstein, S.Popescu and B.Schumacher, Phys. Rev. A \textbf{53}, 2046 (1996).
\bibitem{bennett5} Bennett, C.H., D.P.DiVincenzo, J.A.Smolin and W.K.Wootters, Phys. Rev. A \textbf{54}, 3824 (1996).
\bibitem{bose1} Bose, S., V.Vedral and P.L.Knight, Phys. Rev. A \textbf{57}, 822 (1998).
\bibitem{braunstein1} Braunstein, S.L., V.Buzek and M.Hillery, Phys. Rev. A \textbf{63}, 052313 (2001).
\bibitem{bruss1} Bruss, D., A.Ekert and C.Macchiavello, Phys. Rev. Lett. \textbf{81}, 2598 (1998).
\bibitem{bruss2} Bruss, D., D.P.DiVincenzo, A.Ekert, C.A.Fuchs, C.Macchiavello and J.A.Smolin, Phys. Rev. A \textbf{57},
2368 (1998).
\bibitem{bruss3} Bruss, D. and C.Macchiavello, Phys. Lett. A \textbf{253}, 249 (1999).
\bibitem{bruss4} Bruss, D., G.M.D'Ariano, C.Macchiavello, and M.F.Sacchi, Phys. Rev. A \textbf{62}, 62302 (2000).
\bibitem{bruss5} Bruss, D., J.Calsamiglia and N.Lutkenhaus, Phys. Rev. A \textbf{63}, 042308 (2001).
\bibitem{bruss6} Bruss, D., M.Cinchetti, G.M.D'Ariano and C.Macchiavello, Phys. Rev. A \textbf{62}, 12302 (2000).
\bibitem{bruss7} Bruss, D. and C.Macchiavello, J. Phys. A: Math. Gen. \textbf{34}, 6815 (2001).
\bibitem{bruss8} Bruss, D. and C.Macchiavello, Found. Phys.\textbf{33}, 1617 (2003).
\bibitem{buscemi1} Buscemi, F., G.M.D'Ariano and C.Macchiavello, Phys. Rev. A \textbf{71}, 042327 (2005).
\bibitem{buzek1}  Buzek, V., and M. Hillery, Phys. Rev. A \textbf{54}, 1844 (1996).
\bibitem{buzek2} Buzek, V., V.Vedral, M.B.Plenio, P.L.Knight and M.Hillery, Phys. Rev. A \textbf{55}, 3327 (1997).
\bibitem{buzek3} Buzek, V., S.L.Braunstein, M.Hillery, D.Bruss, Phys. Rev. A \textbf{56}, 3446 (1997).
\bibitem{buzek4}  Buzek, V., and M. Hillery, Phys. Rev. Lett. \textbf{81}, 5003 (1998).
\bibitem{buzek6}  Buzek, V., M. Hillery, and R.Bednik, Acta Phys. Slov. \textbf{48}, 177 (1998).
\bibitem{buzek5} Buzek, V., M. Hillery and R. F. Werner, Phys. Rev. A \textbf{60}, R2626 (1999).
\bibitem{cabello1} Cabello, A., Phys. Rev. A \textbf{61}, 052312 (2000).
\bibitem{cerf5} Cerf, N.J., Acta Phys. Slov. \textbf{48}, 115 (1998).
\bibitem{cerf1} Cerf, N.J., Phys. Rev. Lett. \textbf{84}, 4497 (2000).
\bibitem{cerf2} Cerf, N.J., J. Mod. Opt. \textbf{47}, 187 (2000).
\bibitem{cerf4} Cerf, N.J., T.Durt, and N.Gisin, J. Mod. Opt. \textbf{49}, 1355 (2002).
\bibitem{cerf3} Cerf, N.J., and J.Fiurasek, e-print quant-ph/0512172.
\bibitem{chefles1} Chefles, A. and S.M.Barnett, Phys. Rev. A \textbf{60}, 136 (1999).
\bibitem{chen1} Chen, K., S.Albeverio and S-M Fei, Phys. Rev. Lett. \textbf{95}, 210501 (2005).
\bibitem{chiara1} Chiara, G.D., R.Fazio, C.Macchiavello, S.Montangero and G.M.Palma, Phys. Rev. A \textbf{70}, 062308 (2004).
\bibitem{chiara2} Chiara, G.D., R.Fazio, C.Macchiavello, S.Montangero and G.M.Palma, Phys. Rev. A \textbf{72}, 012328 (2005).
\bibitem{chiribella1} Chiribella, G., G.M.D'Ariano, and P.Perinotti, Phys. Rev. A \textbf{72}, 042336 (2005).
\bibitem{d'ariano2} D'Ariano, G.M., and H.P.Yuen, Phys. Rev. Lett. \textbf{76}, 2832 (1996).
\bibitem{d'ariano1} D'Ariano, G.M., and P.L.Presti, Phys. Rev. A \textbf{64}, 042308 (2001).
\bibitem{deutsch1} Deutsch, D., A.Ekert, R.Jozsa, C.Macchiavello, S.Popescu and A.Sanpera,
Phys. Rev. Lett. \textbf{77}, 2818 (1996).
\bibitem{dobrzanski1} Demkowicz-dobrzanski, R., M.Lewenstein, A.Sen(De), U.Sen, and D.Bruss, Phys. Rev. A \textbf{73}, 032313 (2006).
\bibitem{derka1} Derka, R., V.Buzek and A.Ekert, Phys. Rev. Lett. \textbf{80}, 1571 (1998).
\bibitem{duan1} Duan, L.M., and G.C.Guo, Phys. Rev. Lett. \textbf{80}, 4999 (1998).
\bibitem{duan2} Duan, L.M., G-C Guo, Phys. Rev. A \textbf{64},  054101 (2001).
\bibitem{duan3} Duan, L.M., G-C Guo, e-print quant-ph/9704020.
\bibitem{durt1} Durt, T., and J.Du, Phys. Rev. A \textbf{69}, 062316 (2004).
\bibitem{durt2} Durt, T., J.Fiurasek, and N.J.Cerf, Phys. Rev. A \textbf{72}, 052322 (2005).
\bibitem{ekert1} Ekert, A., Phys. Rev. Lett. \textbf{67}, 661 (1991).
\bibitem{einstein1} Einstein, A., B.Podolsky, and N.Rosen, Phys. Rev. \textbf{47}, 777 (1935).
\bibitem{eisert1} Eisert, J. and M.B.Plenio, J. Mod. Opt. \textbf{46}, 145 (1999).
\bibitem{fan1} Fan, H., X-B Wang, and K.Matsumoto, e-print quant-ph/0012033.
\bibitem{fan2} Fan, H., K.Matsumoto, and M.Wadati, Phys. Rev. A \textbf{64}, 064301 (2001).
\bibitem{fan3} Fan, H., K.Matsumoto, X-B Wang, and M.Wadati, Phys. Rev. A \textbf{65}, 012304 (2002).
\bibitem{fan4} Fan, H., H.Imai, K.Matsumoto, and X-B Wang, Phys. Rev. A \textbf{67}, 022317 (2003).
\bibitem{fan5} Fan, H., Phys. Rev. A \textbf{68}, 054301 (2003).
\bibitem{fan6} Fan, H., B.Liu, and K.Shi, e-print quant-ph/0601017.
\bibitem{fei1} Fei, S-M., Z-X Wang and H.Zhao, Phys. Lett. A \textbf{329}, 414 (2004).
\bibitem{feng1} Feng, J., Y-F Gao, J-S Wang, and M-S Zhan, Phys. Rev. A \textbf{65}, 052311 (2002).
\bibitem{filip2} Filip, R., Phys. Rev. A \textbf{65}, 062320 (2002)
\bibitem{filip1} Filip, R., e-print quant-ph/0401036.
\bibitem{fiurasek1} Fiurasek, J., S.Iblisdir, S.Massar, and N.J.Cerf, Phys. Rev. A \textbf{65}, 040302(R) (2002).
\bibitem{fiurasek2} Fiurasek, J., Phys. Rev. A \textbf{70}, 032308 (2004).
\bibitem{fiurasek3} Fiurasek, J., R.Filip, and N.J.Cerf, Quan. Inf. Comp. \textbf{5}, 583 (2005).
\bibitem{fuchs1} Fuchs, C., N.Gisin, R.B.Griffiths, C.S.Niu, and A.Peres, Phys. Rev. A \textbf{56}, 1163 (1997).
\bibitem{ghirardi1} Ghirardi, G., A.Rimini, and T.Weber, Lett. Nuovo Cimento \textbf{27}, 293 (1980).
\bibitem{ghirardi2} Ghirardi, G., R.Grassi, A.Rimini, and T.Weber, Europhys. Lett. \textbf{6}, 95 (1988).
\bibitem{ghiu1} Ghiu, I., Phys. Rev. A \textbf{67}, 012323 (2003).
\bibitem{ghosh1} Ghosh, S., G.Kar, and A.Roy, Phys. Lett. A \textbf{261}, 17 (1999).
\bibitem{ghosh2} Ghosh, S., G.Kar, S.Kunkri and A.Roy, e-print quant-ph/0312045.
\bibitem{gisin5} Gisin, N., Phys. Lett. A \textbf{154}, 201 (1991).
\bibitem{gisin1} Gisin, N., and S. Massar, Phys. Rev. Lett. \textbf{79}, 2153 (1997).
\bibitem{gisin4} Gisin, N., and B. Hutner, Phys. Lett. A \textbf{228}, 13 (1997).
\bibitem{gisin2} Gisin, N., Phys. Lett. A \textbf{242}, 1 (1998).
\bibitem{gisin3} Gisin, N.,  and S. Popescu, Phys. Rev. Lett. \textbf{83}, 432 (1999).
\bibitem{goldenberg1} Goldenberg, L., and L.Vaidman, Phys. Rev. Lett. \textbf{75}, 1239 (1995).
\bibitem{gorbachev1} Gorbachev, V.N., A.I.Trubilko, A.A.Rodichkina, Phys. Lett. A \textbf{314} (2003) 267.
\bibitem{greenberger1} Greenberger, D.M., M.A.Horne, A.Shimony, and A.Zeilinger, Amer. J. Phys. \textbf{58}, 1131 (1990).
\bibitem{hardy1} Hardy, L., and D. D. Song, Phys. Lett. A \textbf{259}, 331 (1999).
\bibitem{han1} Han, Y-J., Y-S Zhang and G.C.Guo, e-print quant-ph/0209094.
\bibitem{herbert1} Herbert, N., Found. Phys. \textbf{12}, 1171 (1982).
\bibitem{hillery1} Hillery, M., and V.Buzek, Phys. Rev. A \textbf{56}, 1212 (1997).
\bibitem{horo1} Horodecki, M., R. Horodecki, A. Sen(De) and U. Sen, e-print quant-ph/0306044.
\bibitem{horo2} Horodecki, M., P.Horodecki, R.Horodecki, Phys. Lett. A \textbf{223}, 1 (1996).
\bibitem{horo4} Horodecki, M., P.Horodecki, R.Horodecki, Phys. Rev. Lett. \textbf{80}, 5239 (1998).
\bibitem{horo3} Horodecki, M., P.Horodecki, R.Horodecki and M.Piani, e-print quant-ph/0506174.
\bibitem{iblisdir1} Iblisdir, S., A.Acin, N.J.Cerf, R.Filip, J.Fiurasek and N.Gisin, Phys. Rev. A \textbf{72}, 042328 (2005).
\bibitem{iblisdir2} Iblisdir, S., A.Acin, and N.Gisin, e-print quant-ph/0505152.
\bibitem{ishizaka1} Ishizaka, S. and T.Hiroshima, Phys. Rev. A \textbf{62}, 022310 (2000).
\bibitem{jozsa1} Jozsa, R., e-print quant-ph/0204153.
\bibitem{karimipour1} Karimipour, V., and A.T.Rezakhani, Phys. Rev. A \textbf{66}, 052111 (2002).
\bibitem{karpov1} Karpov, E., P.Navez, and N.J.Cerf, Phys. Rev. A \textbf{72}, 042314 (2005).
\bibitem{keyl1} Keyl, M., and R.F.Werner, J. Math. Phys. \textbf{40}, 3283 (1999).
\bibitem{kent1} Kent, A., N.Linden and S.Massar, Phys. Rev. Let.
\textbf{83}, 2656 (1999).
\bibitem{Kwek1} Kwek, L. C., C.H.Oh, X-B Wang and Y.Yeo, Phys. Rev. A \textbf{62}, 052313 (2000).
\bibitem{lamoureux1} Lamoureux, L.-P., and N.J.Cerf, Quan. Inf. Com. \textbf{5}, 032 (2005).
\bibitem{lamoureux2} Lamoureux, L.-P., P.Navez, J.Fiurasek, and N.J.Cerf, Phys. Rev. A \textbf{69}, 040301(R) (2004).
\bibitem{land1} Landauer, R., Physics Today \textbf{44(5}), 22 (1991).
\bibitem{lee1} Lee, S., D.P.Chi, S.D.Oh and J.Kim, Phys. Rev. A \textbf{68}, 062304 (2003).
\bibitem{li1} Li, C., H-S Song and L.Zhou, Journal of Optics B: Quantum semiclass. opt. \textbf{5}, 155
(2003).
\bibitem{maruyama1} Maruyama, K., and P.L. Knight, e-print quant-ph/0309167.
\bibitem{masiak1} Masiak, P., and P.L. Knight, Fortsch. Phys. \textbf{49}, 1001 (2001).
\bibitem{massar1} Massar,S., S.Popescu, Phys. Rev. Lett. \textbf{74}, 1259 (1995).
\bibitem{miranowicz1} Miranowicz, A. and A.Grudka, J. Opt. B: Quantum Semiclass. Optics \textbf{6}, 542
(2004).
\bibitem{navez1} Navez, P., and N.J.Cerf, Phys. Rev. A \textbf{68}, 032313 (2003).
\bibitem{nielsen1} Nielsen, M.A., e-print quant-ph/0011064.
\bibitem{nielsen2} Nielsen, M.A., and I.L.Chuang, Cambridge University Press, Cambridge, 2000.
\bibitem{niu1} Niu, C-S., and R.B.Griffiths, Phys. Rev. A \textbf{58}, 4377 (1998).
\bibitem{niu2} Niu, C-S., and R.B.Griffiths, Phys. Rev. A \textbf{60}, 2764 (1999).
\bibitem{osborne1} Osborne, T.J., Phys. Rev. A \textbf{72}, 022309
(2005).
\bibitem{ozawa1} Ozawa, M., Phys. Lett. A \textbf{268}, 158 (2000).
\bibitem{pati1} Pati, A. K., e-print quant-ph/9908017.
\bibitem{pati2} Pati, A. K., Phys. Rev. Lett. \textbf{83}, 2849 (1999).
\bibitem{pati3} Pati, A. K., Phys. Rev. A \textbf{61}, 022308 (2000).
\bibitem{pati4} Pati, A. K., Phys. Lett. A \textbf{270}, 103 (2000).
\bibitem{pati5} Pati, A. K., and S. L. Braunstein, Nature \textbf{404}, 164 (2000).
\bibitem{pati6} Pati, A. K., and S. L. Braunstein, e-print quant-ph/0007121.
\bibitem{pati7} Pati, A. K., Phys. Lett. A \textbf{270}, 103 (2000).
\bibitem{pati8} Pati, A. K., Phys. Rev. A \textbf{66}, 062319 (2002).
\bibitem{pati9} Pati, A. K., and S. L. Braunstein, Phys. Lett. A \textbf{315}, 208 (2003).
\bibitem{pati10} Pati, A. K., and S. L. Braunstein, e-print quant-ph/0303124.
\bibitem{pati11} Pati, A. K., Fluc. and Noise Lett. \textbf{4}, R27 (2004).
\bibitem{peres1} Peres, A., Phys. Rev. Lett. \textbf{77}, 1413 (1996).
\bibitem{peres2} Peres, A., Phys. Rev. A \textbf{61}, 022117 (2000).
\bibitem{plenio1} Plenio, M.B. and V.Vedral, Contemp. Phys. \textbf{39}, 431
(1998).
\bibitem{qiu1} Qiu, D., Phys. Lett. A \textbf{301}, 112 (2002).
\bibitem{qiu2} Qiu, D., Phys. Rev. A \textbf{65}, 052329 (2002).
\bibitem{qiu3} Qiu, D., Phys. Lett. A \textbf{308}, 335 (2003).
\bibitem{rastegin1} Rastegin, A.E., e-print quant-ph/0208159.
\bibitem{rastegin2} Rastegin, A.E., Phys. Rev. A \textbf{67}, 012305 (2003).
\bibitem{rastegin3} Rastegin, A.E., Phys. Rev. A \textbf{68}, 032303 (2003).
\bibitem{roy1} Roy, A., A.Sen(De) and U.Sen, Phys. Lett. A \textbf{286}, 1 (2001).
\bibitem{scarani1} Scarani, V., S.Iblisdir and N.Gisin, Rev. Mod. Phys. \textbf{77}, 1225 (2005).
\bibitem{scherer1} Scherer, H., and P.Busch, Phys. Rev. A \textbf{47}, 1647 (1993).
\bibitem{shor1} Shor, P.W., and J.Preskill, Phys. Rev. Lett. \textbf{85}, 441 (2000).
\bibitem{song1} Song, D.D., and L.Hardy, e-print quant-ph/0001105.
\bibitem{song2} Song, W., M.Yang and Z-L Cao, Phys. Lett. A \textbf{327}, 123 (2004).
\bibitem{ting1} Ting, G., Y.Feng-Li and W.Zhi-Xi, Chinese Phys.Lett. \textbf{21}, 995 (2004).
\bibitem{vedral1} Vedral.V, M.B.Plenio, M.A.Rippin and P.L.Knight, Phys. Rev. Lett. \textbf{78}, 2275 (1997).
\bibitem{vedral2} Vedral.V and M.B.Plenio, Phys. Rev. A \textbf{57}, 1619 (1998).
\bibitem{vidal1} Vidal. G and R.Tarrach, Phys. Rev. A \textbf{59}, 141 (1999).
\bibitem{vidal2} Vidal. G and R.F.Werner, Phys. Rev. A \textbf{65}, 032314 (2002).
\bibitem{verstraete1} Verstraete, F., K.Audenaert, J.Dehaene and B.D.Moor, J. Phys. A: Math. Gen. \textbf{34}, 10327 (2001).
\bibitem{werner2} Werner, R.F., Phys. Rev. A \textbf{40}, 4277 (1989).
\bibitem{werner1} Werner, R.F., Phys. Rev. A \textbf{58}, 1827 (1998).
\bibitem{wigner1} Wigner, E.P., The logic of personal knowledge: Essays presented to Michael Polany on his
Seventieth birthday, (Routledge and Kegan Paul, London)
\textbf{231} (1961).
\bibitem{wootters1} Wootters, W.K., and W. H. Zurek, Nature \textbf{299}, 802 (1982).
\bibitem{wootters2} Wootters, W.K., Phys. Rev. Lett. \textbf{80}, 2245 (1998).
\bibitem{ying1} Ying, M., Phys. Lett. A \textbf{299}, 107 (2002).
\bibitem{ying2} Ying, M., Phys. Lett. A \textbf{302}, 1 (2002).
\bibitem{yuen1} Yuen, H.P., Phys. Lett. A  \textbf{113}, 405 (1986).
\bibitem{zanardi1} Zanardi, P., Phys. Rev. A \textbf{58}, 3484 (1998).
\bibitem{zhang1} Zhang, C-W., Z-Y Wang, C-F Li and G-C Guo, Phys. Rev. A \textbf{61}, 062310 (2000).
\bibitem{zhang2} Zhang, C-W., C-F Li and G-C Guo, Phys. Lett. A \textbf{271}, 31 (2000).
\bibitem{zhang3} Zhang, C-W., C-F Li and G-C Guo, e-print quant-ph/9908002.
\bibitem{zhang4} Zhang, C-W., C-F Li, Z-Y Wang and G-C Guo, Phys. Rev. A \textbf{62}, 042302 (2000).
\bibitem{zhou1} Zhou, D., B. Zeng, and L. You, Phys. Lett. A \textbf{352}, 41 (2006).
\bibitem{zukowski1} Zukowski, M., A.Zeilinger, M.A.Horne and A.K.Ekert, Phys. Rev. Lett. \textbf{71}, 4287 (1993).
\bibitem{zurek1} Zurek, W. H., Nature \textbf{404}, 130 (2000).
\end{thebibliography}
\end{document}

